Secret key authentication capacity region, Part II: typical authentication rate

This paper investigates the secret key authentication capacity region. Specifically, the focus is on a model where a source must transmit information over an adversary controlled channel where the adversary, prior to the source's transmission, decides whether or not to replace the destination's observation with an arbitrary one of their choosing (done in hopes of having the destination accept a false message). To combat the adversary, the source and destination share a secret key which they may use to guarantee authenticated communications. The secret key authentication capacity region here is then defined as the region of jointly achievable message rate, authentication rate, and key consumption rate (i.e., how many bits of secret key are needed). This is the second of a two part study, with the studies separated by how the authentication rate is measured. Here, the authentication rate is measured by the minimum of the maximum probability of false acceptance where the minimization is over all highly probable subsets of observations at the adversary. That is, consider the maximum probability of false authentication as a function of the adversary's observation, and the adversary's observation as a random variable. The authentication rate is then measured as the smallest number for which the probability that the maximum probability of false authentication is greater than said number is arbitrary small. This is termed typical authentication, since it only needs to consider adversarial observations which are typical with the transmission. Under this measure of authentication matching inner and outer bounds are determined.

==> app_conv.tex <==

\section{Proof of Lemma~\ref{lem:c:2}}\label{app:c}



{\textcolor{purple}{Add note since combination.}}

Before proving Lemma~\ref{lem:c:2} a technical lemma will be useful.
This technical lemma allows for us to bound the probability that, given a correct key, Gr{\'i}ma could fool Bob. 





\begin{lemma}\label{lem:pre:c:2}
If $(f,\varphi)$ is a $(r,\alpha,\kappa,\delta,n)$ code for DM-AIC$(p_{Y|X},p_{Z|X})$, then
$$ \Pr \left( \tau(K,M,S) < 1 - \sqrt{\tilde \delta }\right) \leq \sqrt{\tilde \delta}  $$
where
\begin{align*}
\tau(k,m,s) &\defn \sum_{\mbf{y} : (\mbf{y},k,s) \in \mcf{D}^+ } p(\mbf{y}|k,s)  \varphi(\mcf{M}-\{m\}|\mbf{y},k),
\end{align*} 
and $\tilde \delta = ?.$


\end{lemma}

\subsection{Proof of Lemma~\ref{lem:pre:c:2}}\label{app:pre:c:2:proof}
\begin{IEEEproof}
That
\begin{align}
1-\epsilon &\leq \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\\mbf{y} &\in \mbcf{Y} }} p(\mbf{y},k,m)   \varphi(m|\mbf{y},k)  
%\\&
= \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S} }} p(\mbf{y},k,m,s)   \varphi(m|\mbf{y},k) \label{eq:pre:c:2:start}
\end{align}
follows by the definition of being a $(r,\alpha,\kappa,\epsilon,n)$-TA code and the law of total probability.  
From Equation~\eqref{eq:pre:c:2:start} also follows that 
\begin{align}
1-\tilde \epsilon &\leq \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\ s &\in \mcf{S} }}  p(s,k,m)   \tau(s,k,m)  \label{eq:pre:c:2:middle}
\end{align}
by subtracting $\sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M}\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}, \\ m' &\in \mcf{M} }}  p(\mbf{y},k,m,s)  [p_{M|K,S}(m'|k,s) \varphi(m'|\mbf{y},k)]$ from both sides of Equation~\eqref{eq:pre:c:2:start} and then the properties of the partitioning random variable $S$ and the definition of a decoder to construct the upper bounds
\begin{align*}
&\sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }} p(\mbf{y},k,m,s) p_{M|K,S}(m'|k,s)  [ \varphi(m|\mbf{y},k) -\varphi(m'|\mbf{y},k)] \\
&\leq \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }} p(\mbf{y},k,m,s) p_{M|K,S}(m'|k,s)   \varphi(\{m\} - \{m'\}|\mbf{y},k)\\
%&\leq \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M}\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }} p(\mbf{y},k,m,s) p_{M|K,S}(m'|k,s)   \varphi(\mcf{M} - \{m'\}|\mbf{y},k) \\
&\leq \sum_{\subalign{k&\in \mcf{K},\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }} p(\mbf{y},k,s) p_{M|K,S}(m'|k,s)   \varphi(\mcf{M} - \{m'\}|\mbf{y},k) \\
&\leq \sum_{\subalign{k&\in \mcf{K},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }} \sum_{\mbf{y} \in \mbcf{Y}:(\mbf{y},k,s) \notin \mcf{D}^+} p(\mbf{y},k,s) p(m'|k,s) + \sum_{\subalign{k&\in \mcf{K},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }}  p_{K,M,S}(k,m',s)  \tau(k,m',s) \\
&\leq \lambda_n + \sum_{\subalign{k&\in \mcf{K},\\ s &\in \mcf{S}, \\ m'&\in \mcf{M} }}  p_{K,M,S}(k,m',s)  \tau(k,m',s)
\end{align*}
and
\begin{align*}
& \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M}\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}, \\ m' &\in \mcf{M} }} p(\mbf{y},k,m,s)    p_{M|K,S}(m'|k,s) \varphi(m'|\mbf{y},k) \notag\\
&\leq \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M}\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S} }}  p(\mbf{y},k,m,s) p_{M|K,S}(m|k,s)  + \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M}\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S}  }}  p(\mbf{y},k,m,s)   \varphi(\mcf{M}-\{m\}|\mbf{y},k) \\
&\leq \sum_{(k,m,\mbf{y},s) \in \mcf{D}^+}  p(\mbf{y},k,m,s) 2^{-n(r-\nu_n)}  +\sum_{(k,m,\mbf{y},s) \notin \mcf{D}^+}  p(\mbf{y},k,m,s) + \left[ 1 - \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M}\\\mbf{y} &\in \mbcf{Y},\\ s &\in \mcf{S},  }}  p(\mbf{y},k,m,s)   \varphi(m|\mbf{y},k) \right] \\
&\leq  2^{-n(r-\nu_n)} + \lambda_n + \epsilon. %\label{eq:pre:c:2:startc}
\end{align*}

At the same time a derivation similar to that of Markov's inequality provides
\begin{align}
\sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\ s &\in \mcf{S} }}  p(s,k,m)   \tau(s,k,m) & \leq \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\ s &\in \mcf{S} }}  p(s,k,m) (1-\sqrt{\tilde \epsilon})\idc{ \tau(s,k,m) \leq 1-\sqrt{\tilde \epsilon}} \notag \\
&\hspace{10pt} + \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\ s &\in \mcf{S} }}  p(s,k,m) \left( 1 - \idc{\tau(s,k,m) \leq 1 - \sqrt{\tilde \epsilon}}\right)   \\
&= 1 - \sqrt{\tilde \epsilon} \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\ s &\in \mcf{S} }}  p(s,k,m) \idc{ \tau(s,k,m) \leq 1-\sqrt{\tilde \epsilon}} \label{eq:pre:c:2:final}.
\end{align}


Combining Equations~\eqref{eq:pre:c:2:middle} and~\eqref{eq:pre:c:2:final} then solving for $ \sum_{\subalign{k&\in \mcf{K},\\ m&\in \mcf{M},\\ s &\in \mcf{S} }}  p(s,k,m) \idc{ \tau(s,k,m) \leq 1-\sqrt{\tilde \epsilon}}$ proves the lemma. 
\end{IEEEproof}

\subsection{Proof of $\alpha \leq n^{-1}\mathbb{I}(\mbf{Y};K) + \zeta(\epsilon,n)$}
\begin{IEEEproof}
Suppose $(f,\varphi)$ is a $(r,\alpha,\kappa,\epsilon,n)$-TA code for DM-AIC$(p_{Y|X},p_{Z|X})$. 
By definition a $(r,\alpha,\kappa,\epsilon,n)$-TA code requires
\begin{align}
\epsilon &\geq \max_{\psi \in \mbcf{P}(\mbcf{Y}|\mbcf{Z})} \Pr \left(  \sum_{\mbf{y}\in \mbcf{Y}} \psi(\mbf{y}|\mbf{Z}) \varphi(\mcf{M}-\{M\}|\mbf{y},K) \geq 2^{-n\alpha}  \right)  \\
&\geq  \Pr \left(  \sum_{\mbf{y}\in \mcf{Y}} p_{\mbf{Y}}(\mbf{y})  \varphi(\mcf{M}-\{M\}|\mbf{y},K) \geq 2^{-n\alpha}  \right)  \label{eq:lem:c:2:codeass}
%&=  \sum_{k \in \mcf{K}, m \in \mcf{M}} \Pr \left(  \sum_{\mbf{y}\in \mcf{Y}} p_{\mbf{Y}}(\mbf{y})  \varphi(\mcf{M}-\{m\}|\mbf{y},k) \geq 2^{-n\alpha}  \right) p_{S,K,M}(k,m) 
\end{align}
since $p_{\mbf{Y}} \in \mbcf{P}(\mbcf{Y}|\mbcf{Z})$.
Now, introducing the partitioning random variable from~\cite{graves2018inducing}, $S$, into the RHS of~\eqref{eq:lem:c:2:codeass} provides
\begin{align}
\epsilon &\geq  \sum_{\subalign{k &\in \mcf{K},\\ m &\in \mcf{M},\\ s &\in \mcf{S}}}  \Pr \left(  \sum_{ \tilde s\in \mcf{S}} p(\tilde s) \sum_{\mbf{y} \in \mbcf{Y}} p(\mbf{y}|\tilde s)  \varphi(\mcf{M}-\{m\}|\mbf{y},k) \geq 2^{-n\alpha}  \right)  p(k,m,s)\\
&\geq  \sum_{\subalign{k &\in \mcf{K},\\ m &\in \mcf{M},\\ s &\in \mcf{S}}}  \idc{  p(s) \sum_{\mbf{y} \in \mbcf{Y}: (\mbf{y},k,s) \in \mcf{D}^+} p(\mbf{y}| s)  \varphi(\mcf{M}-\{m\}|\mbf{y},k) \geq 2^{-n\alpha}  }  p(k,m,s)\label{eq:lem:c:2:withs},
\end{align}
where $\mcf{D}^+$ is the stabilized set discussed in Section~\ref{sec:inducing}, since all summands inside the indicator are positive.
Now the partitioning random variable becomes useful as 
\begin{align}
p(\mbf{y}|s) = \frac{p(\mbf{y}|s)}{p(\mbf{y}|k,s)} p(\mbf{y}|k,s) \geq 2^{-\mathbb{I}(\mbf{Y};K|S=s) - 2n\nu_n} p(\mbf{y}|k,s)\label{eq:lem:c:2:withs2}
\end{align}
for all $(\mbf{y},k,s) \in \mcf{D}^+.$
Hence, 
\begin{align}
\epsilon &\geq     \sum_{\subalign{k &\in \mcf{K},\\ m &\in \mcf{M},\\ s &\in \mcf{S}}}   \idc{  2^{-\mathbb{I}(\mbf{Y};K|S=s)-2n\nu_n}  p(s) \tau(k,m,s)  \geq 2^{-n\alpha}  } p(k,m,s) \label{eq:lem:c:2:ssetup}
\end{align}
by combining Equations~\eqref{eq:lem:c:2:withs} and~\eqref{eq:lem:c:2:withs2}; and furthermore
\begin{align}
\epsilon + \sqrt{\tilde \epsilon} &\geq     \sum_{\subalign{ s &\in \mcf{S}}}   \idc{  2^{-\mathbb{I}(\mbf{Y};K|S=s)-2n\nu_n}  p(s) (1-\sqrt{\tilde \epsilon})  \geq 2^{-n\alpha}  } p(s) \label{eq:lem:c:2:ssetup2}
\end{align}
by making use of Lemma~\ref{lem:pre:c:2} and that
\begin{align*}
&  \idc{  2^{-\mathbb{I}(\mbf{Y};K|S=s)-2n\nu_n}  p(s) \tau(k,m,s)  \geq 2^{-n\alpha}  } \\
&\quad\geq  \idc{  2^{-\mathbb{I}(\mbf{Y};K|S=s)-2n\nu_n}  p(s)(1-\sqrt{\tilde \epsilon})  \geq 2^{-n\alpha}  } - \idc{  \tau(k,m,s) < 1 - \sqrt{\tilde \epsilon}} .
\end{align*}

Equation~\eqref{eq:lem:c:2:ssetup2} provides a bound on the number of partitions $s$ for which $\mathbb{I}(\mbf{Y};K|S=s)$ can be less than $n\alpha$.
With this in mind, observe that
\begin{align}
&\mathbb{I}(\mbf{Y};K) + 2 \mathbb{H}(S) + 2n\nu_n -\logt(1-\sqrt{\tilde \epsilon}) \notag \\
&\quad \geq \sum_{s \in \mcf{S}} p(s) \left[ \mathbb{I}(\mbf{Y};K|S=s) - \logt p(s) + 2n\nu_n -\logt(1-\sqrt{\tilde \epsilon})\right]  \\
&\quad \geq \sum_{s \in \mcf{S}} p(s) n\alpha \idc{ 2^{- \mathbb{I}(\mbf{Y};K|S=s)-2n\nu_n }p(s)(1-\sqrt{\tilde \epsilon}) < 2^{-n\alpha}}  \\
&\quad \geq n\alpha( 1 - \epsilon - \sqrt{\tilde \epsilon}), \label{eq:lem:c:2:fin1} 
\end{align}
where~\eqref{eq:lem:c:2:fin1} is where Equation~\eqref{eq:lem:c:2:ssetup2} is specifically used. 
Collecting all the vanishing terms in Equation~\eqref{eq:lem:c:2:fin1} yields 
\begin{align}
\mathbb{I}(\mbf{Y};K) + \zeta(\epsilon,n) & \geq n\alpha \label{eq:lem:c:2:fin} 
\end{align}
where
$$\zeta(\epsilon,n) = \frac{ (\epsilon+ \sqrt{\tilde \epsilon}) |\mcf{Y}| + 2 \nu_n + 2n^{-1} \mathbb{H}(S) - n^{-1} \logt (1-\sqrt{\tilde \epsilon})}{1 - \epsilon - \sqrt{\tilde \epsilon}}.$$
This proves the lemma since $\lim_{\subalign{\epsilon &\rightarrow 0 +,\\ n&\rightarrow \infty}} \zeta(\epsilon,n) = 0  .$

\end{IEEEproof}

\subsection{Proof of $\alpha \leq n^{-1} \mathbb{H}(K|\mbf{Z}) + \zeta(\epsilon,n)$}\label{app:c:1}

\begin{IEEEproof}
Suppose $(f,\varphi)$ is a $(r,\alpha,\kappa,\epsilon,n)$-TA code for DM-AIC$(p_{Y|X},p_{Z|X})$. 
By definition a $(r,\alpha,\kappa,\epsilon,n)$-TA code requires
\begin{align}
\epsilon &\geq \max_{\psi \in \mbcf{P}(\mbcf{Y}|\mbcf{Z})} \Pr \left(  \sum_{\mbf{y}\in \mbcf{Y}} \psi(\mbf{y}|\mbf{Z}) \varphi(\mcf{M}-\{M\}|\mbf{y},K) \geq 2^{-n\alpha}  \right)  \\
&\geq  \Pr \left(  \sum_{\mbf{y}\in \mcf{Y}} \sum_{\subalign{k' &\in \mcf{K},\\ s' &\in \mcf{S}}} p_{\mbf{Y}|K,S}(\mbf{y}|k',s') p_{K,S|\mbf{Z}}(k',s'|\mbf{Z})  \varphi(\mcf{M}-\{M\}|\mbf{y},K) \geq 2^{-n\alpha}  \right)  \label{eq:lem:c:1:codeass} \\
&\geq  \Pr \left(  \sum_{\mbf{y}\in \mcf{Y}:(\mbf{y},k,s) \in \mcf{D}^+} p_{\mbf{Y}|K,S}(\mbf{y}|K,S) p_{K,S|\mbf{Z}}(K,S|\mbf{Z})  \varphi(\mcf{M}-\{M\}|\mbf{y},K) \geq 2^{-n\alpha}  \right) \\
%&=  \Pr \left( p(K,S|\mbf{Z}) \tau(S,K,M)  \geq 2^{-n\alpha}  \right) \\
&=  \sum_{\subalign{\mbf{z} &\in \mbcf{Z}, \\ k & \in \mcf{K}, \\ m&\in \mcf{M}, \\ s &\in \mcf{S}}} \idc{ p(k,s|\mbf{z}) \tau(s,k,m)  \geq 2^{-n\alpha}  } p(\mbf{z},k,m,s) \label{eq:lem:c:1:codeass2}
\end{align}
since $\sum_{\subalign{k' &\in \mcf{K},\\ s' &\in \mcf{S}}} p_{\mbf{Y}|K,S}(\mbf{y}|k',s') p_{K,S|\mbf{Z}}(k',s'|\mbf{Z}) \in \mbcf{P}(\mbcf{Y}|\mbcf{Z})$.
Next, the properties of the partitioning random variable in cooperation with Lemma~\ref{lem:pre:c:2} can be used to find further requirements.  
Specifically, these provide $p(k|\mbf{z},s) \geq 2^{-\mathbb{H}(K|\mbf{Z},S=s) - n\nu_n}$ and $\tau(s,k,m) \geq 1 - \sqrt{\tilde \epsilon}$ for all $(\mbf{z},k,m,s)$ that do not satisfy the low probability events $\tau(s,k,m) < 1-\sqrt{\tilde \epsilon}$ and $(\mbf{z},k,m,s) \notin \mcf{D}^+$.
To make effective use of these properties, recognize that 
\begin{align*} 
\idc{ p(k,s|\mbf{z}) \tau(s,k,m)  \geq 2^{-n\alpha}  } &\geq \idc{ 2^{-\mathbb{H}(K|\mbf{Z},S=s)-n \nu_n} p(s|\mbf{z}) (1-\sqrt{\tilde \epsilon})  \geq 2^{-n\alpha}  } \\
&\quad - \idc{ \tau(s,k,m) < 1-\sqrt{\tilde \epsilon}} - \idc{(\mbf{z},k,m,s) \notin \mcf{D}^+} .
\end{align*}
Hence
\begin{align}
\epsilon + \sqrt{\tilde \epsilon} + \lambda_n &\geq  \sum_{\subalign{\mbf{z} &\in \mbcf{Z}, \\s &\in \mcf{S}}} \idc{ 2^{-\mathbb{H}(K|\mbf{Z},S=s)-n\nu_n} p(s|\mbf{z}) (1-\sqrt{\tilde \epsilon})  \geq 2^{-n\alpha}  }  p(\mbf{z},s) \label{eq:lem:c:1:codeimp2}
\end{align}
because $\Pr \left( \tau(S,K,M) < 1 - \sqrt{\tilde \epsilon}\right) \leq \sqrt{\tilde \epsilon}$ by Lemma~\ref{lem:pre:c:2} while $\Pr \left( (\mbf{Z},K,M,S) \notin \mcf{D}^+ \right) \leq \lambda_n $ by properties of the partitioning random variable. 


Equation~\eqref{eq:lem:c:1:codeimp2}, along with basic information inequalities, yields the following bound
\begin{align}
&\mathbb{H}(K|\mbf{Z}) + \mathbb{H}(S|\mbf{Z},K) + n\nu_n - \logt( 1 - \sqrt{\tilde \epsilon}) \notag \\
&= \sum_{\subalign{\mbf{z} & \in \mbcf{Z},\\s &\in \mcf{S}}} \left[ \mathbb{H}(K|\mbf{Z},S=s) + n\nu_n -\logt p(s|\mbf{z}) - \logt(1-\sqrt{\tilde \epsilon}) \right] p(\mbf{z},s) \\
&\geq \sum_{\subalign{\mbf{z} &\in \mbcf{Z}, \\s &\in \mcf{S}}} n \alpha \idc{ 2^{-\mathbb{H}(K|\mbf{Z},S=s)-n\nu_n} p(s|\mbf{z}) (1-\sqrt{\tilde \epsilon})  < 2^{-n\alpha}  }    p(\mbf{z},s) \\
&\geq n\alpha( 1 - \epsilon - \sqrt{\tilde \epsilon} - \lambda_n)  \label{eq:lem:c:1:fin}
\end{align}
where~\eqref{eq:lem:c:1:fin} makes use of Equation~\eqref{eq:lem:c:1:codeimp2}.
Hence 
\begin{align}
\mathbb{H}(K|\mbf{Z}) + \zeta(\epsilon,n)
&\geq n\alpha \label{eq:lem:c:1:finnish}
\end{align}
where
$$\zeta(\epsilon,n) = \frac{ (\epsilon+ \sqrt{\tilde \epsilon} + \lambda_n) \kappa +  \nu_n + n^{-1} \mathbb{H}(S) - n^{-1} \logt (1-\sqrt{\tilde \epsilon})}{1 - \epsilon - \sqrt{\tilde \epsilon} -\lambda_n}.$$
This proves the lemma since $\lim_{\subalign{\epsilon &\rightarrow 0^+\\ n&\rightarrow \infty}} \zeta(\epsilon,n) = 0  .$





\end{IEEEproof}






\begin{comment}
The following technical lemma will assist in the proof of Lemma~\ref{lem:c:2}.
\begin{lemma}\label{lem:teclemma1}
If $a: \mathbb{R} \rightarrow \mathbb{R}$ is a non-negative function, $p\in \mcf{P}(\mcf{X})$, and $\mcf{X}'\subseteq \mcf{X}$, such that $p_X(\mcf{X}') = \frac{1}{1+\delta} \leq 1$, then
$$\sum_{x \in \mcf{X}'} 2^{-a(x)}p(x) \geq  (1+\delta) 2^{-(1+\delta)\mathbb{E}[a(X)] } .$$

\end{lemma}
\begin{IEEEproof}

In essence the proof is completed by recognizing that $\sum_{x\in \mcf{X}'} \frac{p(x)}{p(\mcf{X}')} = 1$, and using Jensen's inequality. 
More specifically, 
\begin{align}
\sum_{x \in \mcf{X}'} 2^{-a(x)} p(x) & \geq \frac{1}{p(\mcf{X}')} 2^{- \sum_{x \in \mcf{X}'} a(x) \frac{p(x)}{p(\mcf{X}')}} \label{eq:teclemma1:1}\\
& = (1+\delta) 2^{-(1+\delta) \left[\mathbb{E}[a(X)] -\sum_{x \in \mcf{X} - \mcf{X}'} a(x) p(x)  \right]}\\
& \geq (1+\delta) 2^{-(1+\delta) \mathbb{E}[a(X)] } \label{eq:teclemma1:2},
\end{align}
where~\eqref{eq:teclemma1:1} is Jensen's inequality; and~\eqref{eq:teclemma1:2} is because $a$ is non-negative. 
\end{IEEEproof}
\end{comment}

==> app_conv2.tex <==




\begin{comment}

\begin{IEEEproof}

It is sufficient to prove
\begin{equation}\label{eq:lem:c:2:-1}
\mathbb{I}(p_{Y^n|K},p_{K}) > n \alpha \left(1 - \frac{2\sqrt{\delta}+\sqrt{\epsilon}}{1 - 2^{-nr}} \right) - \sqrt{\delta} -\sqrt{\epsilon} - 2^{-nr},
\end{equation}
in order to verify the Lemma. Equation~\eqref{eq:lem:c:2:stat} is a consesuence of substituting $1/2$ for $2^{-nr}$ in Equation~\eqref{eq:lem:c:2:-1}, and solving for $\alpha$ using the bound $n^{-1} \mathbb{I}(p_{Y^n|K},p_{K}) < \abs{\mcf{Y}}$. Equation~\eqref{eq:lem:c:2:-1} follows because, as we will show, 
\begin{equation}\label{eq:lem:c:2:0}
\gamma_1^{-1} + \gamma_2^{-1} + \delta  > \sum_{ y^n, k}  p(y^n,k) \idc{ \frac{p(y^n)}{p(y^n|k) } > 2^{-n \alpha}[1-\gamma_1\epsilon - \gamma_2 \delta - 2^{-nr}]^{-1}}
\end{equation}
for all $(r,\alpha,\kappa,\epsilon,\delta,n)$-TA codes, $\gamma_1 \in (0,(1-2^{-nr})\epsilon^{-1})$ and $\gamma_2 \in (0 , (1-2^{-nr})\delta^{-1})$. Indeed, for then $\mathbb{I}(p_{Y^n|K},p_{K})$ can be bounded as follows
\begin{align*}
\mathbb{I}(p_{Y^n|K},p_{K}) &= \sum_{y^n,k} p(y^n,k) \logt \frac{p(y^n|k)}{p(y^n)} \\
&\geq \sum_{y^n,k  } p(y^n,k)  \idc{\frac{p(y^n)}{p(y^n|k) } \leq 2^{-n \alpha}(1 - 2^{-nr})^{-1}(1-\sqrt{\delta} - \sqrt{\epsilon})^{-1}} \left( n\alpha - \sqrt{\epsilon} - \sqrt{\delta} - 2^{-nr} \right) \\
&\geq \left( n\alpha - \sqrt{\epsilon} - \sqrt{\delta} - 2^{-nr} \right) \left( 1 - \frac{2\sqrt{\delta}+\sqrt{\epsilon}}{1 - 2^{-nr}} \right),
\end{align*}
where the last inequality comes from selecting $\gamma_1 =\frac{1-2^{-nr}}{ \sqrt{\epsilon} }$ and $\gamma_2 = \frac{1-2^{-nr}}{ \sqrt{\delta} }$ in Equation~\eqref{eq:lem:c:2:0}. 

Now to verify Equation~\eqref{eq:lem:c:2:0}, which comes from resuiring both reliability and authenticity, since $\psi$ may be chosen to be $p_{Y^n}$, and thus 
\begin{equation}\label{eq:lem:c:2:1}
\omega_{f,\varphi} (p_{Y^n},z^n,m,k) = \sum_{y^n}   \frac{p(y^n)}{p(y^n|k)}  p(y^n|k)  \left[ \varphi(\mcf{M}|y^n,k) - \varphi(m|y^n,k) \right],
\end{equation}
by extension. Define the following sets 
\begin{align}
\mcf{A} &\defn \set{m,k : \max_{z^n} \omega_{f,\varphi}(p_{Y^n},z^n,m,k) \leq 2^{-n \alpha}  }\\
\mcf{B} &\defn \set{y^n,k : p_{M,K|K}(\mcf{A}|k)  > 1- \gamma_1 \delta }\\
\mcf{C} &\defn \set{y^n,k: \varphi(\mcf{M}|y^n,k) > 1 -\gamma_2 \epsilon }\\
\mcf{D} &\defn \set{y^n,k:  \frac{p(y^n)}{p(y^n|k)} \left[  1 - \gamma_1 \delta - \gamma_2 \epsilon - 2^{-nr} \right] >  2^{-n \alpha}  }.
\end{align}
Demonstrating that 
\begin{align}
%p_{K,M}(\mcf{A})   &\geq 1 - \delta \label{eq:lem:c:2:c1}\\
p_{Y^n,K}(\mcf{B}) &\geq 1 - \gamma_1^{-1} \label{eq:lem:c:2:c2}\\
p_{Y^n,K}(\mcf{C}) &\geq 1 -\gamma_2^{-1} \label{eq:lem:c:2:c3}\\
p_{Y^n,K}(\mcf{B} \cap \mcf{C} \cap \mcf{D}) &\leq \delta  \label{eq:lem:c:2:c4},
\end{align}
proves Equation~\eqref{eq:lem:c:2:0}, hence the Lemma, since 
\begin{align*}
&\sum_{k,y^n}p(k,y^n) \idc{ \frac{p(y^n)}{p(y^n|k)}  >  2^{-n \alpha} \left[  1 - \gamma_1 \delta - \gamma_2 \epsilon - 2^{-nr} \right]^{-1}  }  \\
&=p_{Y^n,K}(\mcf{D}) \\
&\leq 1 - p_{Y^n,K}(\mcf{B} \cap \mcf{C}) + p_{K,Y^n}(\mcf{B}\cap \mcf{C} \cap \mcf{D} )\\
&\leq \gamma_1^{-1} + \gamma_2^{-1} + \delta.
\end{align*}

Equations~\eqref{eq:lem:c:2:c2} and~\eqref{eq:lem:c:2:c3} are a direct result of the definition of $(r,\alpha,\kappa,\epsilon,\delta,n)$-TA codes combined with Markov's inequality. In more detail, Equation~\eqref{eq:lem:c:2:c2} follows because
\begin{equation}
\delta > \sum_{z^n,m,k} p(z^n,m,k) \idc{\omega_{f,\varphi}(p_{Y^n},z^n,m,k) > 2^{-n\alpha}} = \sum_{m,k} p(m,k) \idc{ (m,k) \notin \mcf{A}} = 1 - p_{M,K}(\mcf{A})
\end{equation}
by definition of a $(r,\alpha,\kappa,\epsilon,\delta,n)$-TA code, hence
\begin{equation}
p_{Y^n,K}(\mcf{B}) + ( 1 - p_{Y^n,K}(\mcf{B}))( 1 -\gamma_1 \delta) \geq p_{M,K}(\mcf{A}) > 1 - \delta.
\end{equation}
Similarly for Equation~\eqref{eq:lem:c:2:c3},
\begin{equation}
1- \epsilon < \sum_{y^n,m,k} p (y^n,m,k) \varphi(m|y^n,k) \leq  \sum_{y^n,k} p(y^n,k) \varphi(\mcf{M}|y^n,k)
\end{equation}
by the definition of a $(r,\alpha,\kappa,\epsilon,\delta,n)$-TA code, and hence
\begin{equation}
p_{Y^n,K}(\mcf{C}) + ( 1 - p_{Y^n,K}(\mcf{C}))( 1 -\gamma_1 \epsilon)  \geq \sum_{y^n,k} p(y^n,k) \varphi(\mcf{M}|y^n,k) > 1 - \epsilon.
\end{equation}
On the other hand, to validate Equation~\eqref{eq:lem:c:2:c4}, first observe that 
\begin{equation}\label{eq:lem:c:2:2}
\delta > \sum_{z^n,m,k} p(z^n,m,k) \idc{\omega_{f,\varphi}(p_{Y^n},z^n,m,k) > 2^{-n \alpha }} > \sum_{(m,k) \in \mcf{A}} p(m,k) \max_{z^n} \omega_{f,\varphi}(p_{Y^n},z^n,m,k)  2^{n \alpha }
\end{equation}
since $\max_{z^n} \omega_{f,\varphi}(p_{Y^n},z^n,m,k) < 2^{-n \alpha}$ for all $(m,k) \in \mcf{A}$. Thus, 
\begin{equation}
2^{-n \alpha } \delta  \geq \sum_{k,y^n} p(y^n,k)\frac{p(y^n)}{p(y^n|k)}  \left[ \varphi(\mcf{M}|y^n,k) p_{K,M|K}(\mcf{A}|k) - \sum_{m: (m,k) \in \mcf{A}} 2^{-nr} \varphi(m|y^n,k) \right]
\end{equation}
comes from plugging Equation~\eqref{eq:lem:c:2:1} into the RHS of Equation~\eqref{eq:lem:c:2:2} and performing the summation over $m$. It also follows, then, that 
\begin{align}
2^{-n \alpha } \delta  &\geq \sum_{(k,y^n) \in \mcf{B}\cap \mcf{C} \cap \mcf{D} } p(y^n,k)\frac{p(y^n)}{p(y^n|k)}  \notag \\
&\times \hspace{10pt} \left[ \varphi(\mcf{M}|y^n,k) p_{M,K|K}(\mcf{A}|k) - \sum_{m: (m,k) \in \mcf{A}} 2^{-nr} \varphi(m|y^n,k) \right]
\end{align}
since all summands are positive. But if $(k,y^n) \in \mcf{B}\cap \mcf{C} \cap \mcf{D}$, then
\begin{align}
&\frac{p(y^n)}{p(y^n|k)}  \left[ \varphi(\mcf{M}|y^n,k) p_{M,K|K}(\mcf{A}|k) - \sum_{m: (m,k) \in \mcf{A}} 2^{-nr} \varphi(m|y^n,k) \right] \notag \\
&\geq \frac{p(y^n)}{p(y^n|k)} \left[(1 - \gamma_1\delta)(1-\gamma_2\epsilon) - 2^{-nr}\right]\\
&\geq 2^{-n \alpha}. \label{eq:lem:c:2:sp}
\end{align}
Plugging back into Equation~\eqref{eq:lem:c:2:sp}, then
\begin{equation}
2^{-n \alpha} \delta \geq \sum_{(k,y^n) \in \mcf{B}\cap \mcf{C} \cap \mcf{D} } p(y^n,k) 2^{-n\alpha},
\end{equation}
hence Equation~\eqref{eq:lem:c:2:c4}.

\end{IEEEproof}



\end{comment}


\begin{comment}

\begin{IEEEproof}
Once again, it is sufficient to show
\begin{equation}\label{eq:app:conv:1.1.-1}
\mathbb{H}(p_{K|Z^n}|p_{Z^n}) > n \alpha \left(1 - \delta - \frac{\sqrt{\epsilon}}{1 - 2^{-nr}} \right) -\sqrt{\epsilon} - 2^{-nr}
\end{equation}
to prove the lemma since $\mathbb{H}(p_{K}) = \mathbb{H}(p_{K|Z^n} p_{Z^n}) = n\kappa$ and $\alpha < \abs{\mcf{Y}} + \theta_1(\abs{\mcf{Y}},\epsilon,\delta,n)$ by Lemma~\ref{lem:c:2}. 
Equation~\eqref{eq:app:conv:1.1.-1} is because, as we will show, 
\begin{equation}\label{eq:app:conv:1.1.0}
\delta + \gamma^{-1} > \sum_{ z^n, k}  p(z^n,k) \idc{ p(k|z^n) > 2^{-n \alpha} ( 1 - \gamma\epsilon - 2^{-nr})^{-1} }
\end{equation}
for all $(r,\alpha,\kappa,\epsilon,\delta,n)$-TA codes, and $\gamma \in (0,(1-2^{-nr})\epsilon^{-1})$. Indeed, selecting $\gamma =\frac{1-2^{-nr}}{ \sqrt{\epsilon} }$, observe that 
\begin{align}
\mathbb{H}(p_{K|Z^n}) &= -\sum_{z^n, k} p(z^n,k) \logt p(k|z^n) \notag \\
&\geq \sum_{z^n, k} p(z^n,k) \idc{p(k|z^n) \leq 2^{-n\alpha} (1 - 2^{-nr})(1-\sqrt{\epsilon}) } (n \alpha + \logt ( 1-\sqrt{\epsilon}) + \logt ( 1 - 2^{-nr}) ) \notag \\
&\geq \sum_{z^n, k} p(z^n,k) \idc{p(k|z^n) \leq 2^{-n\alpha} (1 - 2^{-nr})(1-\sqrt{\epsilon}) } (n \alpha-\sqrt{\epsilon} - 2^{-nr})  \notag \\
&\geq \left(1 - \delta - \frac{\sqrt{\epsilon}}{1 - 2^{-nr}} \right) (n \alpha - \sqrt{\epsilon} - 2^{-nr}). \notag
\end{align}


Thus, we seek to validate Equation~\eqref{eq:app:conv:1.1.0}. To do this, note 
\begin{equation}\label{eq:app:conv:1.1.1}
\delta > \max_{\psi} \sum_{ z^n,m, k} p(z^n,m,k) \idc{\omega(\psi,z^n,m,k) > 2^{-n \alpha}}
\end{equation}
by definition of a $(r,\alpha,\kappa,\epsilon,\delta,n)$-TA codes.
Any choice of $\psi$ must be less than or equal to the maximum, so in particular choose 
\[
\psi(y^n|z^n) \defn \sum_{k, m} p(k|z^n) \abs{\mcf{M}}^{-1} \idc{y^n = y^n_{m,k}},
\]
where $y^n_{i,j} \in \mcf{Y}^n$ is a sequence for which $\varphi(i| y^{n}_{i,j},j) \geq 1 - \varepsilon_{f,\varphi}(i,j)$. Define the set 
\[
\mcf{A} := \set{ z^n,k : \min_{m} \omega_{f,\varphi}(\psi,z^n,m,k) \geq  p(k|z^n) ( 1 - \gamma \epsilon - 2^{-n r} ) },
\]
and, for the moment, assume that $p_{Z^n,K}(\mcf{A}) \geq 1 - \gamma^{-1}$. Equation~\eqref{eq:app:conv:1.1.0} directly follows from this assumption since 
\begin{align}
\delta &> \sum_{ z^n,m, k} p(z^n,m,k) \idc{\omega_{\varphi}(\psi,z^n,m,k) > 2^{-n \alpha}} \notag \\
&\geq \sum_{(z^n,k) \in \mcf{A} } \sum_{m} p(z^n,m,k) \idc{p(k|z^n) ( 1 - \gamma\epsilon - 2^{-n r})  > 2^{-n \alpha}}\notag \\
&\geq -\gamma^{-1} + \sum_{z^n,k } p(z^n,k) \idc{p(k|z^n) ( 1 - \gamma\epsilon - 2^{-n r})  > 2^{-n \alpha}}.
\end{align}


Returning to the assumption $p_{Z^n,K}(\mcf{A}) \geq 1 - \gamma^{-1}$, first, $\omega_{f,\varphi}(\psi,z^n,m,k)$ can be bounded as follows,
\begin{align}
\omega_{f,\varphi}(\psi,z^n,m,k)&= \sum_{(k',m') \in \mcf{K}\times \mcf{M}} p_{K|Z^n}( k'|z^n) \abs{\mcf{M}}^{-1} \varphi(\mcf{M} - \set{m,\mbf{!}} | y_{m', k'}^n, k) \notag \\
&\geq p(k |z^n) \sum_{ m' \in \mcf{M}} \abs{\mcf{M}}^{-1} \varphi(\mcf{M} - \set{m,\mbf{!}} | y_{m', k}^n, k) \notag \\
&\geq p(k |z^n) \sum_{ m' \in \mcf{M} -\set{ m} } \abs{\mcf{M}}^{-1} \varphi( m' | y_{m', k}^n,  k)  \notag \\
&\geq p(k |z^n) \left( -2^{-n r } + \sum_{ m'\in \mcf{M}} \abs{\mcf{M}}^{-1} [1 - \varepsilon_{f,\varphi}(m',k)]  \right).
\end{align}
Thus, the probability of $\mcf{A}$ is greater than the probability of a selecting a $k$ uniformly at random, such that 
\[
\sum_{ m \in \mcf{M}} \abs{\mcf{M}}^{-1} [1 - \varepsilon_{f,\varphi}(m,k)]   > 1 - \gamma \epsilon.
\]
Therefore, $p_{Z^n,K}(\mcf{A}) \geq 1 - \gamma^{-1}$ follows by Markov's inequality and that by definition  
\[
1- \varepsilon_{f,\varphi} = \sum_{k,m} \abs{\mcf{K}}^{-1} \abs{\mcf{M}}^{-1} [1 - \varepsilon_{f,\varphi}(m,k)] = 1 - \varepsilon_{f,\varphi} > 1-\epsilon.
\]
\end{IEEEproof}

\end{comment}
